Damping of the isovector giant dipole resonance in $^{40,48}$Ca

The fine structure of the IsoVector Giant Dipole Resonance (IVGDR) in the doubly-magic nuclei $^{40,48}$Ca observed in inelastic proton scattering experiments under $0^\circ$ is used to investigate the role of different mechanisms contributing to the IVGDR decay width. Characteristic energy scales are extracted from the fine structure by means of wavelet analysis. The experimental scales are compared to different theoretical approaches allowing for the inclusion of complex configurations beyond the mean-field level. Calculations are performed in the framework of RPA and beyond-RPA in a relativistic approach based on an effective meson-exchange interaction, with the UCOM effective interaction and, for the first time, with realistic two- plus three-nucleon interactions from chiral effective field theory employing the in-medium similarity renormalization group. All models highlight the role of Landau fragmentation for the damping of the IVGDR, while the differences in the coupling strength between one particle-one hole (1p-1h) and two particle-two hole (2p-2h) correlated (relativistic) and non-correlated (non-relativistic) configurations lead to very different pictures of the importance of the spreading width resulting in wavelet scales being a sensitive measure of their interplay. The relativistic approach with particle-vibration coupling, in particular, shows impressive agreement with the number and absolute values of the scales extracted from the experimental data.

==> References.tex <==
\bibitem{har01}
M. N. Harakeh and A. van der Woude, Giant Resonances:
Fundamental High-Frequency Modes of Nuclear Excitation (Oxford University, Oxford, 2001).

\bibitem{bbb98}
P.F. Bortignon, A. Bracco, R.A. Broglia, Giant Resonances: Nuclear Structure at Finite Temperature (Harwood Academic, Amsterdam, 1998).

\bibitem{bol88}
G.O. Bolme, L.S. Cardman, R. Doerfler, L.J. Koester Jr., B.L. Miller, C.N. Papanicolas, H. Rothhaas, S.E. Williamson, Phys. Rev. Lett. 61 (1988) 1081.

\bibitem{die94}
H. Diesener, U. Helm, G. Herbert, V. Huck, P. von Neumann-Cosel, C. Rangacharyulu, A. Richter, G. Schrieder, A. Stascheck, A. Stiller, J. Ryckebusch, J. Carter,
%
Phys. Rev. Lett. 72 (1994) 1994.

\bibitem{str00} 
S. Strauch, P. von Neumann-Cosel, C. Rangacharyulu, A. Richter, G. Schrieder, K. Schweda, J. Wambach, Phys. Rev. Lett. 85 (2000) 2913.

\bibitem{car01}
J. Carter, H. Diesener, U. Helm, G. Herbert, P. von Neumann-Cosel, A. Richter, G. Schrieder, S. Strauch,
Nucl. Phys. A 696 (2001) 317.

\bibitem{hun03}
M. Hunyadi, A.M. van den Berg, N. Blasi, C. B\"aumer, M. Csatlos, L. Csige, B. Davids, U. Garg, J. Gulyas, M.N. Harakeh, M.A. de Huu, B.C. Junk, A. Krasznahorkay, S. Rakers, D. Sohler, H.J. W\"ortche, Phys. Lett. B 576 (2003) 253.

\bibitem{vnc19a}
P. von Neumann-Cosel, V.Yu. Ponomarev, A. Richter, J. Wambach, Eur. Phys. J. A 55 (2019) 224

\bibitem{she08} 
A. Shevchenko,  J. Carter, G.R.J. Cooper, R.W. Fearick, S.V. F\"{o}rtsch, Y. Kalmykov, P. von Neumann-Cosel, V.Yu. Ponomarev, A. Richter, I. Usman, J. Wambach, Phys. Rev. C 77 (2008) 024302.

\bibitem{pol14} 
I. Poltoratska, R.W. Fearick, A.M. Krumbholz, E. Litvinova, H. Matsubara, P. von Neumann-Cosel, V.Yu. Ponomarev, A. Richter, A. Tamii, Phys. Rev. C 89 (2014) 054322.

\bibitem{fea18}
R.W. Fearick, B. Erler, H. Matsubara, P. von Neumann-Cosel, A. Richter, R. Roth, A. Tamii, Phys. Rev. C 97 (2018) 044325.

\bibitem{jin18} 
M. Jingo, E.Z. Buthelezi, J. Carter, G.R.J. Cooper, R.W. Fearick, S.V. F\"ortsch, C.O. Kureba A.M. Krumbholz, P. von Neumann-Cosel, R. Neveling, P. Papka, I. Poltoratska, V.Yu. Ponomarev, A. Richter, E. Sideras-Haddad, F.D. Smit, J.A. Swartz, A. Tamii, I.T. Usman, Eur. Phys. J. A 54 (2018) 254.

\bibitem{bas20}
S. Bassauer, P. von Neumann-Cosel, P.-G. Reinhard, A. Tamii, S. Adachi, C.A. Bertulani, P.Y. Chan, A. D'Alessio, H. Fujioka, H. Fujita, Y. Fujita, G. Gey, M. Hilcker, T.H. Hoang, A. Inoue, J. Isaak, C. Iwamoto, T. Klaus, N. Kobayashi, Y. Maeda, M. Matsuda, N. Nakatsuka, S. Noji, H.J. Ong, I. Ou, N. Pietralla, V.Yu. Ponomarev, M.S. Reen, A. Richter, M. Singer, G. Steinhilber, T. Sudo, Y. Togano, M. Tsumura, Y. Watanabe, V. Werner, Phys. Rev. C 102 (2020) 034327.

\bibitem{don20}
L.M. Donaldson, J. Carter, P. von Neumann-Cosel, V.O. Nesterenko, R. Neveling, V.Yu. Ponomarev, P.-G. Reinhard, I.T. Usman, P. Adsley, C.A. Bertulani, J.W. Br\"ummer, E.Z. Buthelezi, G.R.J. Cooper, R.W. Fearick, S.V. F\"ortsch, H. Fujita, Y. Fujita, M. Jingo, N.Y. Kheswa, W. Kleinig, C.O. Kureba, J. Kvasil, M. Latif, K.C.W. Li, J.P. Mira, F. Nemulodi, P. Papka, L. Pellegri, N. Pietralla, B. Rebeiro,
A. Richter, N.Yu. Shirikova, E. Sideras-Haddad, A.V. Sushkov, F.D. Smit, G.F. Steyn, J.A. Swartz, A. Tamii, Phys. Rev. C 102 (2020) 064327.

\bibitem{she04} 
A. Shevchenko, J. Carter, R.W. Fearick, S.V. F\"{o}rtsch, H. Fujita, Y. Fujita, Y. Kalmykov, D. Lacroix, J.J. Lawrie, P. von Neumann-Cosel, R. Neveling, V.Yu. Ponomarev, A. Richter, E. Sideras-Haddad, F.D. Smit, J. Wambach, Phys. Rev. Lett. 93 (2004) 122501.

\bibitem{she09} 
A. Shevchenko, O. Burda, J. Carter, G.R.J. Cooper, R.W. Fearick, S.V. F\"{o}rtsch, H. Fujita, Y. Fujita, Y. Kalmykov, D. Lacroix, J.J. Lawrie, P. von Neumann-Cosel, R. Neveling, V.Yu. Ponomarev, A. Richter, E. Sideras-Haddad, F.D. Smit, J. Wambach, Phys. Rev. C 79 (2009) 044305. 

\bibitem{usm11}
I. Usman, Z. Buthelezi, J. Carter, G.R.J. Cooper, R.W. Fearick, S.V. F\"ortsch, H. Fujita, Y. Kalmykov, P. von Neumann-Cosel, R. Neveling, I. Poltoratska, A. Richter, A. Shevchenko, E. Sideras-Haddad, F.D. Smit, and J. Wambach, Phys. Rev. C 84 (2011) 054322.

\bibitem{usm16}
I.T. Usman, Z. Buthelezi, J. Carter, G.R.J. Cooper, R.W. Fearick, S.V. F\"ortsch, H. Fujita, Y. Fujita, P. von Neumann-Cosel, R. Neveling, P. Papakonstantinou, I.~Pysmenetska, A. Richter, R. Roth, E. Sideras-Haddad, F.D. Smit, Phys. Rev. C 94 (2016) 024308.

\bibitem{kur18}
C.O. Kureba,  Z. Buthelezi, J. Carter, G.R.J. Cooper, R.W. Fearick, S.V. F\"ortsch, M. Jingo, W. Kleinig, A. Krugmann, A.M. Krumbholz, J. Kvasil, J. Mabiala, J.P. Mira, V.O. Nesterenko, P. von Neumann-Cosel,  R. Neveling, P. Papka,  P.-G. Reinhard, A. Richter, E. Sideras-Haddad, F.D. Smit, G.F. Steyn, J.A. Swartz, A. Tamii, I.T. Usman, Phys. Lett. B 779 (2018) 269.

\bibitem{vnc19b}
P. von Neumann-Cosel, A. Tamii, Eur. Phys. J A 55 (2019) 110.

\bibitem{dro90}
S. Dro\.{z}d\.{z}, S. Nishizaki, J. Speth, J. Wambach, Phys. Rep. 197 (1990) 1.

\bibitem{pap09}
P. Papakonstantinou, R. Roth, Phys. Lett. B 671 (2009) 356.

\bibitem{pap10}
P. Papakonstantinou, R. Roth, Phys. Rev. C 81 (2010) 024317.

\bibitem{lit08}
E. Litvinova, P. Ring, V. Tselyaev, Phys. Rev. C 78 (2008) 014312; erratum Phys. Rev. C 78 (2008) 049902.

\bibitem{tri16}
R. Trippel, Doctoral thesis D17, TU Darmstadt (2016); https://tuprints.ulb.tu-darmstadt.de/5883.

\bibitem{tam09}
%A. Tamii {\em et al.},
A.~Tamii, Y.~Fujita, H.~Matsubara, T.~Adachi, J.~Carter, M.~Dozono, H.~Fujita, K.~Fujita, H.~Hashimoto, K.~Hatanaka, T.~Itahashi, M.~Itoh, T.~Kawabata, K.~Nakanishi, S.~Ninomiya, A.B.~Perez-Cerdan, L.~Popescu, B.~Rubio, T.~Saito, H.~Sakaguchi, Y.~Sakemi, Y.~Sasamoto, Y.~Shimbara, Y.~Shimizu, F.D.~Smit, Y.~Tameshige, M.~Yosoi, J.~Zenhiro,
%
Nucl. Instrum. Methods A 605 (2009) 3.

\bibitem{nev11} 
R. Neveling, H. Fujita, F.D. Smit, T. Adachi, G.P.A. Berg, E.Z. Buthelezi, J. Carter, J.L. Conradie, M. Couder, R.W. Fearick, S.V. F\"{o}rtsch, D.T. Fourie, Y. Fujita, J. G\"{o}rres, K. Hatanaka, M. Jingo, A.M. Krumbholz, C.O. Kureba, J P. Mira, S.H.T. Murray, P. von Neumann-Cosel, S. O$'$Brien, P. Papka, I. Poltoratska, A. Richter, E. Sideras-Haddad, J.A. Swartz, A. Tamii, I. Usman, J.J. van Zyl,
%
Nucl. Instrum. Methods A 654 (2011) 29; erratum 662 (2012) 101.

\bibitem{lat17}
M. Latif, PhD thesis, University of the Witwatersrand (2017).

\bibitem{don18}
L.M. Donaldson, C.A. Bertulani, J. Carter, V.O. Nesterenko, P. von Neumann-Cosel, R. Neveling, V.Yu Ponomarev, P.-G. Reinhard, I.T. Usman, P. Adsley, J.W. Brummer, E.Z. Buthelezi, G.R.J. Cooper, R.W. Fearick, S.V. F\"ortsch, H. Fujita, Y. Fujita, M. Jingo, W. Kleinig, C.O. Kureba, J. Kvasil, M. Latif, K.C.W. Li, J.P. Mira, F. Nemulodi, P. Papka, L. Pellegri, N. Pietralla, A. Richter, E. Sideras-Haddad, F.D. Smit, G F. Steyn, J.A. Swartz, A. Tamii, 
%
Phys. Lett. B 776 (2018) 133.

\bibitem{bir17}
J. Birkhan, M. Miorelli, S. Bacca, S. Bassauer, C. A. Bertulani, G. Hagen, H. Matsubara, P. von Neumann-Cosel, T. Papenbrock, N. Pietralla, V.Yu. Ponomarev, A. Richter, A. Schwenk, A. Tamii, 
%
Phys. Rev. Lett. 118 (2017) 252501.

\bibitem{kal06} 
Y. Kalmykov, T. Adachi, G.P.A. Berg, H. Fujita, K. Fujita, Y. Fujita, K. Hatanaka, J. Kamiya, A.K. Nakanishi, P. von Neumann-Cosel, V.Yu. Ponomarev, A. Richter, N. Sakamoto, Y. Sakemi, A. Shevchenko, Y. Shimbara, Y. Shimizu, F.D. Smit, T. Wakasa, J. Wambach, M. Yosoi, 
%
Phys. Rev. Lett. 96 (2006) 012502.


%\bibitem{ber88}
 %C. Bertulani and G. Baur, Phys. Rep. 163, 299 (1988).

%\bibitem{ber09}
 %C. Bertulani, arXiv:0908.4307.

\bibitem{ber93}
 C. Bertulani, A. Nathan, Nucl. Phys. A 554 (1993) 158.

\bibitem{ahr75}
J. Ahrens, H. Borchert, K. Czock, H. Eppler, H. Gimm, H. Gundrum, M. Kröning, P. Riehn, G.S. Ram, A. Zieger, B. Ziegler, Nucl. Phys. A 251 (1975) 479.

%%%%%%% RRPA-RTBA %%%%%%%

\bibitem{Vretenar1999}
D. Vretenar, P. Ring, G.A. Lalazissis, N. Paar, Nucl. Phys. A 649 (1999) 29.

\bibitem{Ma2001}
Z.Y. Ma, N. Van Giai, A. Wandelt, D. Vretenar, P. Ring, Nucl. Phys. A 687 (2001) 64.

\bibitem{PaarRingNiksicEtAl2003}
N. Paar, P. Ring, T.{Nik{\v{s}}i{\'c}}, D. Vretenar,
Phys. Rev. C 67 (2003) 034312.

\bibitem{LitvinovaRingTselyaev2007}
E. Litvinova, P. Ring, V. Tselyaev, Phys. Rev. C 75 (2007) 064308.

\bibitem{LitvinovaRingTselyaev2008}
E. Litvinova, P. Ring, V. Tselyaev, Phys. Rev. C 78 (2008) 014312.

\bibitem{LitvinovaRingTselyaev2010}
E. Litvinova, P. Ring, V. Tselyaev, Phys. Rev. Lett. 105 (2010) 022502.

\bibitem{LitvinovaSchuck2019}
E. Litvinova, P. Schuck, Phys. Rev. C 100 (2019) 064320.

\bibitem{LitvinovaLoensLangankeEtAl2009}
E. Litvinova, H. Loens, K. Langanke, G. Martinez-Pinedo, T. Rauscher, P. Ring, F.-K. Thielemann, V. Tselyaev, Nucl. Phys. A 823 (2009) 26.

\bibitem{EndresLitvinovaSavranEtAl2010}
J. Endres, E. Litvinova, D. Savran, P.A. Butler, M.N. Harakeh, S. Harissopulos, R.-D. Herzberg, R. Kr\"ucken, A. Lagoyannis, N. Pietralla, V.Yu. Ponomarev, L. Popescu, P. Ring, M. Scheck, K. Sonnabend, V.I. Stoica, H.J. W\"ortche,
A. Zilges, Phys. Rev. Lett. 105 (2010) 212503.

\bibitem{EndresSavranButlerEtAl2012}
J. Endres, D. Savran, P.A. Butler, M.N. Harakeh, S. Harissopulos, R.-D. Herzberg, R. Kr\"ucken, A. Lagoyannis, E. Litvinova, N. Pietralla, V. Ponomarev, L. Popescu, P. Ring, M. Scheck, F. Schl\"uter, K. Sonnabend, V.I. Stoica, H.J.
W\"ortche, A. Zilges, Phys. Rev. C 85 (2012) 064331.

\bibitem{LanzaVitturiLitvinovaEtAl2014}
E. Lanza, A. Vitturi, E. Litvinova, D. Savran, Phys. Rev. C 89 (2014) 041601.

\bibitem{Oezel-TashenovEndersLenskeEtAl2014}
B. \"Ozel-Tashenov, J. Enders, H. Lenske, A. Krumbholz, E. Litvinova, P. von Neumann-Cosel, I. Poltoratska, A. Richter, G. Rusev, D. Savran, N. Tsoneva, Phys. Rev. C 90 (2014) 024304.

\bibitem{EgorovaLitvinova2016}
I.A. Egorova, E. Litvinova, Phys. Rev. C 94 (2016) 034322.

\bibitem{Lalazissis1997}
G. Lalazissis, J. K\"onig, P. Ring, Phys. Rev. C 55 (1997) 540.

\bibitem{tsu10}
K.~Tsukiyama, S.K. Bogner, A.~Schwenk, Phys. Rev. Lett. 106 (2011) 222502.

\bibitem{her12}
H.~Hergert, S.K. Bogner, S.~Binder, A.~Calci, J.~Langhammer, R.~Roth, A.~Schwenk, Phys. Rev. C 87 (2013) 034307.
  
\bibitem{her15}
H.~Hergert, S.K. Bogner, T.D. Morris, A.~Schwenk, K.~Tsukiyama, Phys. Rep. 621 (2016) 165.
  
\bibitem{pap14}
P.~Papakonstantinou, Phys. Rev. C 90 (2014) 024305.  
\bibitem{tse13}
V.I.~Tselyaev, Phys. Rev. C 88 (2013) 054301.

\bibitem{eks15}
A.~Ekstr\"om, G.R. Jansen, K.A. Wendt, G.~Hagen, T.~Papenbrock, B.D. Carlsson, C.~Forss\'en, M.~Hjorth-Jensen, P.~Navr\'atil, W.~Nazarewicz, Phys. Rev. C 91 (2015) 051301.  
\bibitem{rot14}
R.~Roth, A.~Calci, J.~Langhammer, S.~Binder, Phys. Rev. C 90 (2014) 024325.

\bibitem{coo08}
G.R.J. Cooper, D.R. Cowan, Comput. Geosci. 34 (2008) 95.

%\bibitem{teo98}
%A. Teolis, in Computational Signal Processing with Wavelets (Birkhauser, Boston, 1998) 59.

\bibitem{eck89}
F.J. Eckle, H. Lenske, G. Eckle, G. Graw, R. Hertenberger, H. Kader, F. Merz, H. Nann, P. Schiemenz, H.H. Wolter, Phys. Rev. C 39 (1989) R1662.

\bibitem{gro79}
W. Gross, D. Meuer, A. Richter, E. Spamer, O. Titze, W.Kn\"upfer, Phys. Lett. B 84 (1979) 296.


